RF Power Transmission for Self-sustaining Miniaturized IoT Devices

Radio Frequency (RF) wireless power transfer is a promising technology that has the potential to constantly power small Internet of Things (IoT) devices, enabling even battery-less systems and reducing their maintenance requirements. However, to achieve this ambitious goal, carefully designed RF energy harvesting (EH) systems are needed to minimize the conversion losses and the conversion efficiency of the limited power. For intelligent internet of things sensors and devices, which often have non-constant power requirements, an additional power management stage with energy storage is needed to temporarily provide a higher power output than the power being harvested. This paper proposes an RF wireless power energy conversion system for miniaturized IoT composed of an impedance matching network, a rectifier, and power management with energy storage. The proposed sub-system has been experimentally validated and achieved an overall power conversion efficiency (PCE) of over 30 % for an input power of -10 dBm and a peak efficiency of 57 % at 3 dBm.

==> src/02_RelatedWork.tex <==
\section{Related Work}\label{sec:relatedwork}
% TODO not clear how deep this can be or what makes sense... ideally we manage to get a comparison to some research works...) 
% no related work section due to space constraints

A variety of devices employ WPT such as wireless charging by magnetic resonance [1], [2], for biomedical devices [3], and for electrical vehicles [4].



this is a excellent starign source \cite{Costanzo2021} https://ieeexplore.ieee.org/document/9597599 to write a good introduction
\\RECENT LITERATURE
\\Field:	                    Source
\\Review RF energy transfer	\cite{Clerckx2019}[2]*, \cite{PonnimbadugePerera2018}, \cite{Meile2019}, \cite{Lu2016}
\\Antenna design	            \cite{Wagih2020}, \cite{Eid2020}
\\Rectifier design	        \cite{Park2020}*, \cite{Rotenberg2020}*, \cite{Colaiuda2020}*, \cite{Nimo2015}*, \cite{Liu2020}
\\Application	                \cite{Yedavalli2017}, \cite{Bhamra2021}, \cite{Li2020}, \cite{Pinuela2013}
\\ *highly relevant

